Mitigating the Bias of Centered Objects in Common Datasets

Convolutional networks are considered shift invariant, but it was demonstrated that their response may vary according to the exact location of the objects. In this paper we will demonstrate that most commonly investigated datasets have a bias, where objects are over-represented at the center of the image during training. This bias and the boundary condition of these networks can have a significant effect on the performance of these architectures and their accuracy drops significantly as an object approaches the boundary. We will also demonstrate how this effect can be mitigated with data augmentation techniques.

==> OldFormatTables.tex <==
\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|r|r|r|}
\hline
  \cellcolor[HTML]{C0C0C0}&
  \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}Losses in \\ the center \\ (central 30\% \\ allowed)\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}Losses at \\ the edges \\ (central 70\% \\ forbidden)\end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}Different/Same \\ loss ratio\end{tabular}} \\ \hline
\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}Trained in \\ the center \\ (central 30\% \\ allowed)\end{tabular} &
  0.000411 &
  6.974354 &
  16,086.638 \\ \hline
\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}Trained at \\ the edges \\ (central 70\% \\ forbidden)\end{tabular} &
  0.000690 &
  0.000417 &
  1.898 \\ \hline
\end{tabular}%
}
\caption{This table shows the arithmetic mean values of the losses corresponding to the to the trainings and the evaluations at the center (central 30\% allowed) and at the edges (central 70\% forbidden), as well as the ratios between testing on the same type of data set versus testing on the opposite (in order: ${edge\ test}/{center\ test}$ for center training and ${center\ test}/{edge\ test}$ for edge training) on 5 individually trained neural networks for each case. As the ratios show, the results get worse in both cases if the training and test sets have different object placement patterns, however the increase of loss is far more drastic in case of central training.}\label{tab:M2NIST_ImgNet_03-07Values}
\end{table}


\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{C0C0C0}}r |r|r|r|}
\hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}ForbiddenRegion \\ (central training - \\ forbidden edges)\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.1-0.2 test \\ band region\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.2-0.3 test \\  band region\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.3-0.4 test \\  band region\end{tabular}} \\ \hline
0 & 0.945 & 0.980 & 1.082 \\ \hline
0.1 & 0.917 & 0.963 & 1.008 \\ \hline
0.2 & 0.959 & 0.918 & 0.937 \\ \hline
0.3 & 1.106 & 0.894 & 0.972 \\ \hline
0.4 & 1.308 & 0.891 & 1.012 \\ \hline
0.5 & 0.887 & 0.923 & 0.955 \\ \hline
0.6 & 0.898 & 0.921 & 0.853 \\ \hline
0.7 & 1.036 & 1.032 & 1.061 \\ \hline
0.8 & 1.025 & 1.048 & 1.104 \\ \hline
0.9 & 1.141 & 1.212 & 1.150 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.4-0.5 test \\  band region\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.5-0.6 test \\  band region\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.6-0.7 test \\  band region\end{tabular}} \\ \hline
0 & 0.980 & 1.062 & 1.085 \\ \hline
0.1 & 1.070 & 0.957 & 0.956 \\ \hline
0.2 & 0.889 & 1.055 & 1.028 \\ \hline
0.3 & 0.979 & 0.976 & 1.066 \\ \hline
0.4 & 1.049 & 0.981 & 2.202 \\ \hline
0.5 & 0.947 & 1.048 & 13.921 \\ \hline
0.6 & 0.868 & 0.891 & 17.030 \\ \hline
0.7 & 0.866 & 1.447 & 58.702 \\ \hline
0.8 & 1.125 & 1.018 & 23.522 \\ \hline
0.9 & 1.217 & 1.429 & 69.234 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.7-0.8 test \\  band region\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.8-0.9 test \\  band region\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.9-1.0 test \\  band region\end{tabular}} \\ \hline
0 & 0.987 & 0.989 & 1.041 \\ \hline
0.1 & 1.019 & 0.909 & 1.927 \\ \hline
0.2 & 0.934 & 1.535 & 16.101 \\ \hline
0.3 & 4.315 & 404.340 & 3,164.413 \\ \hline
0.4 & 411.924 & 7,549.861 & 25,575.147 \\ \hline
0.5 & 246.706 & 2,098.795 & 8,063.583 \\ \hline
0.6 & 319.163 & 1,697.250 & 5,924.594 \\ \hline
0.7 & 831.526 & 5,900.890 & 17,408.368 \\ \hline
0.8 & 390.934 & 2,655.341 & 9,557.831 \\ \hline
0.9 & 839.521 & 5,890.076 & 21,579.727 \\ \hline
\end{tabular}
}
\caption{This table shows the arithmetic mean values of training-evaluation pairs on 5 individually trained neural networks for each row. The rows represent the normalized loss values corresponding to the same set of neural networks trained on images with a given "outer" restriction on the object position (the first column marks the ratio of forbidden region near the edges, and thus how tight is the allowed position for the objects around the center of the image) The columns represent the normalized loss values corresponding to the same level of "inner and outer" restriction on the object position during the testing (the first rows for each block mark the closeness of the allowed band to the center of the image, and thus how far the objects must appear from the center of the image). The loss values in the table are normalized by the loss values corresponding to the most central (0.0-0.1) object placements.}\label{tab:M2NIST_ImgNet_ArMeanLosses_Bands}
\end{table}


\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{C0C0C0}}r |r|r|r|}
\hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}ForbiddenRegion \\ (central training - \\ forbidden edges)\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.1 test \\ forbidden center\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.2 test \\ forbidden center\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.3  test \\ forbidden center\end{tabular}} \\ \hline
0 & 0.862 & 0.894 & 0.930 \\ \hline
0.1 & 1.018 & 1.097 & 1.050 \\ \hline
0.2 & 0.869 & 1.116 & 1.063 \\ \hline
0.3 & 1.327 & 1.155 & 1.211 \\ \hline
0.4 & 1.090 & 1.057 & 1.095 \\ \hline
0.5 & 0.902 & 0.906 & 0.877 \\ \hline
0.6 & 0.992 & 1.000 & 0.976 \\ \hline
0.7 & 0.998 & 0.913 & 1.063 \\ \hline
0.8 & 0.975 & 1.053 & 1.014 \\ \hline
0.9 & 1.083 & 1.023 & 1.069 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.4  test \\ forbidden center\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.5  test \\ forbidden center\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.6  test \\ forbidden center\end{tabular}} \\ \hline
0 & 0.984 & 1.029 & 0.832 \\ \hline
0.1 & 1.170 & 1.150 & 1.189 \\ \hline
0.2 & 1.198 & 1.245 & 1.311 \\ \hline
0.3 & 1.265 & 1.493 & 1.565 \\ \hline
0.4 & 1.222 & 1.233 & 1.439 \\ \hline
0.5 & 1.020 & 0.941 & 1.111 \\ \hline
0.6 & 1.002 & 1.065 & 1.180 \\ \hline
0.7 & 1.025 & 1.127 & 1.301 \\ \hline
0.8 & 1.051 & 1.140 & 1.282 \\ \hline
0.9 & 1.075 & 1.243 & 1.344 \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{C0C0C0}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.7  test \\ forbidden center\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.8  test \\ forbidden center\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}NormLossVal \\ 0.9  test \\ forbidden center\end{tabular}} \\ \hline
0 & 1.022 & 1.004 & 1.061 \\ \hline
0.1 & 1.252 & 1.377 & 1.699 \\ \hline
0.2 & 1.486 & 2.090 & 3.237 \\ \hline
0.3 & 1.921 & 2.614 & 4.373 \\ \hline
0.4 & 1.801 & 2.463 & 3.789 \\ \hline
0.5 & 1.421 & 1.904 & 2.975 \\ \hline
0.6 & 1.396 & 1.750 & 2.461 \\ \hline
0.7 & 1.565 & 2.337 & 3.132 \\ \hline
0.8 & 1.500 & 2.061 & 2.925 \\ \hline
0.9 & 1.461 & 1.992 & 3.537 \\ \hline
\end{tabular}
}
\caption{This table shows the arithmetic mean values of training-evaluation pairs on 5 individually trained neural networks for each row. The rows represent the normalized loss values corresponding to the same set of neural networks trained on images with a given "outer" restriction on the object position (the first column marks the ratio of forbidden region near the edges, and thus how tight is the allowed position for the objects around the center of the image). The columns represent the normalized loss values corresponding to the same level of "inner" restriction on the object position during the testing (the first rows for each block mark the ratio of forbidden region near the center of the image, and thus how far the objects must appear from the center of the image). The loss values in the table are normalized by the loss values corresponding to the losses on object positions with no restrictions.}\label{tab:M2NIST_ImgNet_ArMeanLosses_FullRegions}
\end{table}
